A deformation problem for Galois representations over imaginary quadratic fields

We prove the modularity of minimally ramified ordinary residually reducible p-adic Galois representations of an imaginary quadratic field F under certain assumptions. We first exhibit conditions under which the residual representation is unique up to isomorphism. Then we prove the existence of deformations arising from cuspforms on GL_2(A_F) via the Galois representations constructed by Taylor et al. We establish a sufficient condition (in terms of the non-existence of certain field extensions which in many cases can be reduced to a condition on an L-value) for the universal deformation ring to be a discrete valuation ring and in that case we prove an R=T theorem. We also study reducible deformations and show that no minimal characteristic 0 reducible deformation exists.

==> makros.tex <==
%Some Greek letters

\def\a{\alpha}
\def\b{\beta}
\def\g{\gamma}
\def\G{\Gamma}
\def\d{\delta}
\def\D{\Delta}
\def\e{\epsilon}
\def\h{\theta}
\def\k{\kappa}
\def\l{\lambda}
\def\L{\Lambda}
\def\s{\sigma}
\def\S{\Sigma}
\def\o{\omega}
\def\O{\Omega}

%Mathcal

\newcommand{\mA}{\mathcal{A}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mJ}{\mathcal{J}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mQ}{\mathcal{Q}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mU}{\mathcal{U}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mZ}{\mathcal{Z}}


%mathfrak (missing \fi)

\newcommand{\fa}{\mathfrak{a}}
\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fb}{\mathfrak{b}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fc}{\mathfrak{c}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fd}{\mathfrak{d}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fe}{\mathfrak{e}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\ff}{\mathfrak{f}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fh}{\mathfrak{h}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fj}{\mathfrak{j}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fk}{\mathfrak{k}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fl}{\mathfrak{l}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fm}{\mathfrak{m}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fo}{\mathfrak{o}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fr}{\mathfrak{r}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fs}{\mathfrak{s}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\ft}{\mathfrak{t}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fu}{\mathfrak{u}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fv}{\mathfrak{v}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fw}{\mathfrak{w}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fx}{\mathfrak{x}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fy}{\mathfrak{y}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fz}{\mathfrak{z}}
\newcommand{\fZ}{\mathfrak{Z}}


%mathbf

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}


\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{m}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}




%rings of integers (note the different definition of OE), adeles
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\OA}{\mathcal{O}_A}
\newcommand{\OB}{\mathcal{O}_B}
\newcommand{\OC}{\mathcal{O}_C}
\newcommand{\OD}{\mathcal{O}_D}
\newcommand{\Oe}{\mathcal{O}_E}
\newcommand{\OF}{\mathcal{O}_F}
\newcommand{\OG}{\mathcal{O}_G}
\newcommand{\OH}{\mathcal{O}_H}
\newcommand{\OI}{\mathcal{O}_I}
\newcommand{\OJ}{\mathcal{O}_J}
\newcommand{\OK}{\mathcal{O}_K}
\newcommand{\OL}{\mathcal{O}_L}
\newcommand{\OM}{\mathcal{O}_M}
\newcommand{\ON}{\mathcal{O}_N}
\newcommand{\OO}{\mathcal{O}_O}
\newcommand{\OP}{\mathcal{O}_P}
\newcommand{\OQ}{\mathcal{O}_Q}
\newcommand{\OR}{\mathcal{O}_R}
\newcommand{\OS}{\mathcal{O}_S}
\newcommand{\OT}{\mathcal{O}_T}
\newcommand{\OU}{\mathcal{O}_U}
\newcommand{\OV}{\mathcal{O}_V}
\newcommand{\OW}{\mathcal{O}_W}
\newcommand{\OX}{\mathcal{O}_X}
\newcommand{\OY}{\mathcal{O}_Y}
\newcommand{\OZ}{\mathcal{O}_Z}

\newcommand{\Ae}{\mathbf{A}_E}
\newcommand{\AF}{\mathbf{A}_F}
\newcommand{\AK}{\mathbf{A}_K}
\newcommand{\AL}{\mathbf{A}_L}
\newcommand{\AM}{\mathbf{A}_M}
\newcommand{\AN}{\mathbf{A}_N}
\newcommand{\AQ}{\mathbf{A}}
\newcommand{\Aef}{\mathbf{A}_{E,\textup{f}}}
\newcommand{\AFf}{\mathbf{A}_{F,\textup{f}}}
\newcommand{\AKf}{\mathbf{A}_{K,\textup{f}}}
\newcommand{\ALf}{\mathbf{A}_{L,\textup{f}}}
\newcommand{\AMf}{\mathbf{A}_{M,\textup{f}}}
\newcommand{\ANf}{\mathbf{A}_{N,\textup{f}}}
\newcommand{\AQf}{\mathbf{A}_{\textup{f}}}
\newcommand{\Aeu}{\mathbf{A}_E^{\times}}
\newcommand{\AFu}{\mathbf{A}_F^{\times}}
\newcommand{\AKu}{\mathbf{A}_K^{\times}}
\newcommand{\ALu}{\mathbf{A}_L^{\times}}
\newcommand{\AMu}{\mathbf{A}_M^{\times}}
\newcommand{\ANu}{\mathbf{A}_N^{\times}}
\newcommand{\AQu}{\mathbf{A}^{\times}}
\newcommand{\Aefu}{\mathbf{A}_{E,\textup{f}}^{\times}}
\newcommand{\AFfu}{\mathbf{A}_{F,\textup{f}}^{\times}}
\newcommand{\AKfu}{\mathbf{A}_{K,\textup{f}}^{\times}}
\newcommand{\ALfu}{\mathbf{A}_{L,\textup{f}}^{\times}}
\newcommand{\AMfu}{\mathbf{A}_{M,\textup{f}}^{\times}}
\newcommand{\ANfu}{\mathbf{A}_{N,\textup{f}}^{\times}}
\newcommand{\AQfu}{\mathbf{A}_{\textup{f}}^{\times}}


%localizations 

\newcommand{\Oop}{\mathcal{O}_{\mathfrak{p}}}
\newcommand{\mOp}{\mathcal{O}_{\mathfrak{p}}}
\newcommand{\OAp}{\mathcal{O}_{A,\mathfrak{p}}}
\newcommand{\OBp}{\mathcal{O}_{B,\mathfrak{p}}}
\newcommand{\OCp}{\mathcal{O}_{C,\mathfrak{p}}}
\newcommand{\ODp}{\mathcal{O}_{D,\mathfrak{p}}}
\newcommand{\Oep}{\mathcal{O}_{E,\mathfrak{p}}}
\newcommand{\OFp}{\mathcal{O}_{F,\mathfrak{p}}}
\newcommand{\OGp}{\mathcal{O}_{G,\mathfrak{p}}}
\newcommand{\OHp}{\mathcal{O}_{H,\mathfrak{p}}}
\newcommand{\OIp}{\mathcal{O}_{I,\mathfrak{p}}}
\newcommand{\OJp}{\mathcal{O}_{J,\mathfrak{p}}}
\newcommand{\OKp}{\mathcal{O}_{K,\mathfrak{p}}}
\newcommand{\OLp}{\mathcal{O}_{L,\mathfrak{p}}}
\newcommand{\OMp}{\mathcal{O}_{M,\mathfrak{p}}}
\newcommand{\ONp}{\mathcal{O}_{N,\mathfrak{p}}}
\newcommand{\OOp}{\mathcal{O}_{O,\mathfrak{p}}}
\newcommand{\OPp}{\mathcal{O}_{P,\mathfrak{p}}}
\newcommand{\OQp}{\mathcal{O}_{Q,\mathfrak{p}}}
\newcommand{\ORp}{\mathcal{O}_{R,\mathfrak{p}}}
\newcommand{\OSp}{\mathcal{O}_{S,\mathfrak{p}}}
\newcommand{\OTp}{\mathcal{O}_{T,\mathfrak{p}}}
\newcommand{\OUp}{\mathcal{O}_{U,\mathfrak{p}}}
\newcommand{\OVp}{\mathcal{O}_{V,\mathfrak{p}}}
\newcommand{\OWp}{\mathcal{O}_{W,\mathfrak{p}}}
\newcommand{\OXp}{\mathcal{O}_{X,\mathfrak{p}}}
\newcommand{\OYp}{\mathcal{O}_{Y,\mathfrak{p}}}
\newcommand{\OZp}{\mathcal{O}_{Z,\mathfrak{p}}}

\newcommand{\OoP}{\mathcal{O}_{\mathfrak{P}}}
\newcommand{\mOP}{\mathcal{O}_{\mathfrak{P}}}
\newcommand{\OAP}{\mathcal{O}_{A,\mathfrak{P}}}
\newcommand{\OBP}{\mathcal{O}_{B,\mathfrak{P}}}
\newcommand{\OCP}{\mathcal{O}_{C,\mathfrak{P}}}
\newcommand{\ODP}{\mathcal{O}_{D,\mathfrak{P}}}
\newcommand{\OeP}{\mathcal{O}_{E,\mathfrak{P}}}
\newcommand{\OFP}{\mathcal{O}_{F,\mathfrak{P}}}
\newcommand{\OGP}{\mathcal{O}_{G,\mathfrak{P}}}
\newcommand{\OHP}{\mathcal{O}_{H,\mathfrak{P}}}
\newcommand{\OIP}{\mathcal{O}_{I,\mathfrak{P}}}
\newcommand{\OJP}{\mathcal{O}_{J,\mathfrak{P}}}
\newcommand{\OKP}{\mathcal{O}_{K,\mathfrak{P}}}
\newcommand{\OLP}{\mathcal{O}_{L,\mathfrak{P}}}
\newcommand{\OMP}{\mathcal{O}_{M,\mathfrak{P}}}
\newcommand{\ONP}{\mathcal{O}_{N,\mathfrak{P}}}
\newcommand{\OOP}{\mathcal{O}_{O,\mathfrak{P}}}
\newcommand{\OPP}{\mathcal{O}_{P,\mathfrak{P}}}
\newcommand{\OQP}{\mathcal{O}_{Q,\mathfrak{P}}}
\newcommand{\ORP}{\mathcal{O}_{R,\mathfrak{P}}}
\newcommand{\OSP}{\mathcal{O}_{S,\mathfrak{P}}}
\newcommand{\OTP}{\mathcal{O}_{T,\mathfrak{P}}}
\newcommand{\OUP}{\mathcal{O}_{U,\mathfrak{P}}}
\newcommand{\OVP}{\mathcal{O}_{V,\mathfrak{P}}}
\newcommand{\OWP}{\mathcal{O}_{W,\mathfrak{P}}}
\newcommand{\OXP}{\mathcal{O}_{X,\mathfrak{P}}}
\newcommand{\OYP}{\mathcal{O}_{Y,\mathfrak{P}}}
\newcommand{\OZP}{\mathcal{O}_{Z,\mathfrak{P}}}

\newcommand{\Ooq}{\mathcal{O}_{\mathfrak{q}}}
\newcommand{\mOq}{\mathcal{O}_{\mathfrak{q}}}
\newcommand{\OAq}{\mathcal{O}_{A,\mathfrak{q}}}
\newcommand{\OBq}{\mathcal{O}_{B,\mathfrak{q}}}
\newcommand{\OCq}{\mathcal{O}_{C,\mathfrak{q}}}
\newcommand{\ODq}{\mathcal{O}_{D,\mathfrak{q}}}
\newcommand{\Oeq}{\mathcal{O}_{E,\mathfrak{q}}}
\newcommand{\OFq}{\mathcal{O}_{F,\mathfrak{q}}}
\newcommand{\OGq}{\mathcal{O}_{G,\mathfrak{q}}}
\newcommand{\OHq}{\mathcal{O}_{H,\mathfrak{q}}}
\newcommand{\OIq}{\mathcal{O}_{I,\mathfrak{q}}}
\newcommand{\OJq}{\mathcal{O}_{J,\mathfrak{q}}}
\newcommand{\OKq}{\mathcal{O}_{K,\mathfrak{q}}}
\newcommand{\OLq}{\mathcal{O}_{L,\mathfrak{q}}}
\newcommand{\OMq}{\mathcal{O}_{M,\mathfrak{q}}}
\newcommand{\ONq}{\mathcal{O}_{N,\mathfrak{q}}}
\newcommand{\OOq}{\mathcal{O}_{O,\mathfrak{q}}}
\newcommand{\OPq}{\mathcal{O}_{P,\mathfrak{q}}}
\newcommand{\OQq}{\mathcal{O}_{Q,\mathfrak{q}}}
\newcommand{\ORq}{\mathcal{O}_{R,\mathfrak{q}}}
\newcommand{\OSq}{\mathcal{O}_{S,\mathfrak{q}}}
\newcommand{\OTq}{\mathcal{O}_{T,\mathfrak{q}}}
\newcommand{\OUq}{\mathcal{O}_{U,\mathfrak{q}}}
\newcommand{\OVq}{\mathcal{O}_{V,\mathfrak{q}}}
\newcommand{\OWq}{\mathcal{O}_{W,\mathfrak{q}}}
\newcommand{\OXq}{\mathcal{O}_{X,\mathfrak{q}}}
\newcommand{\OYq}{\mathcal{O}_{Y,\mathfrak{q}}}
\newcommand{\OZq}{\mathcal{O}_{Z,\mathfrak{q}}}

\newcommand{\OoQ}{\mathcal{O}_{\mathfrak{Q}}}
\newcommand{\mOQ}{\mathcal{O}_{\mathfrak{Q}}}
\newcommand{\OAQ}{\mathcal{O}_{A,\mathfrak{Q}}}
\newcommand{\OBQ}{\mathcal{O}_{B,\mathfrak{Q}}}
\newcommand{\OCQ}{\mathcal{O}_{C,\mathfrak{Q}}}
\newcommand{\ODQ}{\mathcal{O}_{D,\mathfrak{Q}}}
\newcommand{\OeQ}{\mathcal{O}_{E,\mathfrak{Q}}}
\newcommand{\OFQ}{\mathcal{O}_{F,\mathfrak{Q}}}
\newcommand{\OGQ}{\mathcal{O}_{G,\mathfrak{Q}}}
\newcommand{\OHQ}{\mathcal{O}_{H,\mathfrak{Q}}}
\newcommand{\OIQ}{\mathcal{O}_{I,\mathfrak{Q}}}
\newcommand{\OJQ}{\mathcal{O}_{J,\mathfrak{Q}}}
\newcommand{\OKQ}{\mathcal{O}_{K,\mathfrak{Q}}}
\newcommand{\OLQ}{\mathcal{O}_{L,\mathfrak{Q}}}
\newcommand{\OMQ}{\mathcal{O}_{M,\mathfrak{Q}}}
\newcommand{\ONQ}{\mathcal{O}_{N,\mathfrak{Q}}}
\newcommand{\OOQ}{\mathcal{O}_{O,\mathfrak{Q}}}
\newcommand{\OPQ}{\mathcal{O}_{P,\mathfrak{Q}}}
\newcommand{\OQQ}{\mathcal{O}_{Q,\mathfrak{Q}}}
\newcommand{\ORQ}{\mathcal{O}_{R,\mathfrak{Q}}}
\newcommand{\OSQ}{\mathcal{O}_{S,\mathfrak{Q}}}
\newcommand{\OTQ}{\mathcal{O}_{T,\mathfrak{Q}}}
\newcommand{\OUQ}{\mathcal{O}_{U,\mathfrak{Q}}}
\newcommand{\OVQ}{\mathcal{O}_{V,\mathfrak{Q}}}
\newcommand{\OWQ}{\mathcal{O}_{W,\mathfrak{Q}}}
\newcommand{\OXQ}{\mathcal{O}_{X,\mathfrak{Q}}}
\newcommand{\OYQ}{\mathcal{O}_{Y,\mathfrak{Q}}}
\newcommand{\OZQ}{\mathcal{O}_{Z,\mathfrak{Q}}}

\newcommand{\OAv}{\mathcal{O}_{A,v}}
\newcommand{\OBv}{\mathcal{O}_{B,v}}
\newcommand{\OCv}{\mathcal{O}_{C,v}}
\newcommand{\ODv}{\mathcal{O}_{D,v}}
\newcommand{\Oev}{\mathcal{O}_{E,v}}
\newcommand{\OFv}{\mathcal{O}_{F,v}}
\newcommand{\OGv}{\mathcal{O}_{G,v}}
\newcommand{\OHv}{\mathcal{O}_{H,v}}
\newcommand{\OIv}{\mathcal{O}_{I,v}}
\newcommand{\OJv}{\mathcal{O}_{J,v}}
\newcommand{\OKv}{\mathcal{O}_{K,v}}
\newcommand{\OLv}{\mathcal{O}_{L,v}}
\newcommand{\OMv}{\mathcal{O}_{M,v}}
\newcommand{\ONv}{\mathcal{O}_{N,v}}
\newcommand{\OOv}{\mathcal{O}_{O,v}}
\newcommand{\OPv}{\mathcal{O}_{P,v}}
\newcommand{\OQv}{\mathcal{O}_{Q,v}}
\newcommand{\ORv}{\mathcal{O}_{R,v}}
\newcommand{\OSv}{\mathcal{O}_{S,v}}
\newcommand{\OTv}{\mathcal{O}_{T,v}}
\newcommand{\OUv}{\mathcal{O}_{U,v}}
\newcommand{\OVv}{\mathcal{O}_{V,v}}
\newcommand{\OWv}{\mathcal{O}_{W,v}}
\newcommand{\OXv}{\mathcal{O}_{X,v}}
\newcommand{\OYv}{\mathcal{O}_{Y,v}}
\newcommand{\OZv}{\mathcal{O}_{Z,v}}

\newcommand{\OAw}{\mathcal{O}_{A,w}}
\newcommand{\OBw}{\mathcal{O}_{B,w}}
\newcommand{\OCw}{\mathcal{O}_{C,w}}
\newcommand{\ODw}{\mathcal{O}_{D,w}}
\newcommand{\Oew}{\mathcal{O}_{E,w}}
\newcommand{\OFw}{\mathcal{O}_{F,w}}
\newcommand{\OGw}{\mathcal{O}_{G,w}}
\newcommand{\OHw}{\mathcal{O}_{H,w}}
\newcommand{\OIw}{\mathcal{O}_{I,w}}
\newcommand{\OJw}{\mathcal{O}_{J,w}}
\newcommand{\OKw}{\mathcal{O}_{K,w}}
\newcommand{\OLw}{\mathcal{O}_{L,w}}
\newcommand{\OMw}{\mathcal{O}_{M,w}}
\newcommand{\ONw}{\mathcal{O}_{N,w}}
\newcommand{\OOw}{\mathcal{O}_{O,w}}
\newcommand{\OPw}{\mathcal{O}_{P,w}}
\newcommand{\OQw}{\mathcal{O}_{Q,w}}
\newcommand{\ORw}{\mathcal{O}_{R,w}}
\newcommand{\OSw}{\mathcal{O}_{S,w}}
\newcommand{\OTw}{\mathcal{O}_{T,w}}
\newcommand{\OUw}{\mathcal{O}_{U,w}}
\newcommand{\OVw}{\mathcal{O}_{V,w}}
\newcommand{\OYw}{\mathcal{O}_{Y,w}}
\newcommand{\OZw}{\mathcal{O}_{Z,w}}


%textup commands

\newcommand{\tua}{\textup{a}}
\newcommand{\tuc}{\textup{c}}
\newcommand{\tuf}{\textup{f}}
\newcommand{\tuh}{\textup{h}}
\newcommand{\tum}{\textup{m}}
\newcommand{\tuM}{\textup{M}}

\newcommand{\tualg}{\textup{alg}}
\newcommand{\tucl}{\textup{cl}}
\newcommand{\tucusp}{\textup{cusp}}
\newcommand{\tuDesc}{\textup{Desc}}
\newcommand{\tuint}{\textup{int}}
\newcommand{\tuMaass}{\textup{Maass}}
\newcommand{\tumin}{\textup{min}}
\newcommand{\tumax}{\textup{max}}
\newcommand{\tuNM}{\textup{NM}}
\newcommand{\tuord}{\textup{ord}}
\newcommand{\tus}{\textup{s}}
\newcommand{\tuss}{\textup{ss}}
\newcommand{\tust}{\textup{st}} 
\newcommand{\tuun}{\textup{un}}
\newcommand{\tuuniv}{\textup{univ}}



%Comments
\newcommand{\com}[1]{\vspace{5 mm}\par \noindent
\marginpar{\textsc{Comment}} \framebox{\begin{minipage}[c]{0.95
\textwidth} \tt #1 \end{minipage}}\vspace{5 mm}\par}




%Some mathematical symbols

\newcommand{\ov}{\overline}



%equation environment

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bes}{\begin{equation*}}
\newcommand{\ees}{\end{equation*}}

\newcommand{\bs}{\begin{split}}
\newcommand{\es}{\end{split}}
\newcommand{\bss}{\begin{split*}}
\newcommand{\ess}{\end{split*}}

\newcommand{\bmat}{\left[ \begin{matrix}}
\newcommand{\emat}{\end{matrix} \right]}
\newcommand{\bsmat}{\left[ \begin{smallmatrix}}
\newcommand{\esmat}{\end{smallmatrix} \right]}

\newcommand{\bml}{\begin{multline}}
\newcommand{\eml}{\end{multline}}
\newcommand{\bmls}{\begin{multline*}}
\newcommand{\emls}{\end{multline*}}




%math commands
\newcommand{\tu}{\textup}

%Math operators

\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\BC}{BC}
\DeclareMathOperator{\Card}{Card}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\cond}{cond}
\DeclareMathOperator{\Desc}{Desc}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\disc}{disc}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Fitt}{Fitt}
\DeclareMathOperator{\Frob}{Frob}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\GSp}{GSp}
\DeclareMathOperator{\GU}{GU}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\image}{Im}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\Nm}{Nm}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\ResR}{R}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\restr}{res}
\DeclareMathOperator{\Sel}{Sel}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\Sp}{Sp}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\SU}{SU}
\DeclareMathOperator{\Symm}{Symm^2}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\U}{U}
\DeclareMathOperator{\val}{val}






%Old commands
\def\f{\phi}
\def\p{\psi}
\def\t{\tau}
\def\c{\chi}
\def\qu{\mathbb{Q}}
\def\qub{\ov{\mathbb{Q}}}
\def\quf{\mathbf{Q}}
\def\qufb{\ov{\mathbf{Q}}}
\def\AQf{\mathbf{A}_{\textup{f}}}
\def\ideleF{\mathbf{A}_F^{\times}}
\def\ideleFf{\mathbf{A}_{F,\textup{f}}^{\times}}
\def\adeleF{\mathbf{A}_F}
\def\adeleFf{\mathbf{A}_{F,\textup{f}}}
\def\adele{\mathbf{A}}
\def\idele{\mathbf{A}^{\times}}
\def\adeleQ{\mathbf{A}}
\def\ideleQ{\mathbf{A}^{\times}}
\def\adeleK{\mathbf{A}_K}
\def\ideleK{\mathbf{A}^{\times}_K}
\def\hh{\textup{h}}



%Special commands

\def\bb{\mathbf}
\def\bbf{\mathbf}
%\def\bs{\setminus}
\def\Tpi{T^{\textup{h}}_{\pi}}
\def\Tpio{T^{\textup{h}}_{\pi, 0}}
\def\HK{\mathcal{H}_{K_{0,p}}}
\def\Mmnh{\mathcal{M}^{\textup{nh}}_m(N, \psi)}

\newcommand{\lpr}{\char'40l}
\newcommand{\no}{\noindent}
\newcommand{\R}{\textup{Res}_{K/\mathbf{Q}}\hspace{2pt}}
\newcommand{\sep}{\hspace{3pt} | \hspace{3pt}}
\newcommand{\bi}[1]{\overline{#1}^{-1}}
\newcommand{\ro}[1]{{#1}^{\rho}}
\newcommand{\tbi}[1]{(\bar{#1}^t)^{-1}}
\newcommand{\Ga}{\mathbf{G}_a}
\newcommand{\hs}{\hspace{2pt}}
\newcommand{\hf}{\hspace{5pt}}
%\newcommand{\OKp}{\mathcal{O}_{K,p}}
\newcommand{\OKptwo}{\left(\mathcal{O}_{K,p}\right)^2_2}
\newcommand{\Op}{\mathcal{O}_{(\mathfrak{p})}}
\newcommand{\fpi}{\mathfrak{p}_i}
\newcommand{\iy}{\infty}
\newcommand{\iyr}{\infty\rho}
\newcommand{\I}{\mathbf{i}}
\newcommand{\GhN}{\Gamma_0^{\textup{h}}(N)}
\newcommand{\DhN}{\Delta_0^{\textup{h}}(N)}
\newcommand{\RhN}{R^{\textup{h}}(N)}
\newcommand{\ThN}{\mathbf{T}^{\textup{h}}_{\bfC}(N)}
\newcommand{\ThC}{\mathbf{T}^{\textup{h}}_{\mathbf{C}}}


\newcommand{\tr}{\textup{tr}\hspace{2pt}}
\newcommand{\Ur}{\textup{Im}\hspace{2pt}}
\newcommand{\Rz}{\textup{Re}\hspace{2pt}}
\newcommand{\res}[1]{\textup{res}_{s=#1}\hspace{2pt}}
\newcommand{\uni}[1]{{#1}^{\text{univ}}}
\newcommand{\tm}{\tilde{M}}
\newcommand{\pq}{\psi'_{\mathbf{Q}}}
\newcommand{\pqi}{(\psi'_{\mathbf{Q}})^{-1}}
\newcommand{\cq}{\chi_{\mathbf{Q}}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\invlim}{\mathop{\varprojlim}\limits}
\newcommand{\dirlim}{\mathop{\varinjlim}\limits}




